Multilinear Hyperquiver Representations

We count singular vector tuples of a system of tensors assigned to the edges of a directed hypergraph. To do so, we study the generalisation of quivers to directed hypergraphs. Assigning vector spaces to the nodes of a hypergraph and multilinear maps to its hyperedges gives a hyperquiver representation. Hyperquiver representations generalise quiver representations (where all hyperedges are edges) and tensors (where there is only one multilinear map). The singular vectors of a hyperquiver representation are a compatible assignment of vectors to the nodes. We compute the dimension and degree of the variety of singular vectors of a sufficiently generic hyperquiver representation. Our formula specialises to known results that count the singular vectors and eigenvectors of a generic tensor. Lastly, we study a hypergraph generalisation of the inverse tensor eigenvalue problem and solve it algorithmically.

==> figures/n-periodic-orbit-table.tex <==
\begin{table}
\centering
\resizebox{0.625\columnwidth}{!}
{\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\backslashbox{$n$}{$d$} \multirow{2}{*}{} & \multicolumn{2}{l|}{2} & \multicolumn{2}{l|}{3} & \multicolumn{2}{l|}{4}                                \\ 
\cline{2-7}
                  & $m=3$ & $m=4$             & $m=3$ & $m=4$             & $m=3$ & $m=4$                                                       \\ 
\hline
1                 & 3    & 4               & 7    & 13               & 15    & 40                                                            \\ 
\hline
2                 & 5   & 10               & 21    & 91               & 85    & -                                                        \\ 
\hline
3                 & 9   & 28               & 73    & -              & -    & -                                              \\ 
\hline
4                 & 17    & 82               & -    & -            & -    & -                                            \\ 
\hline
\end{tabular}}
\caption{The degree of the singular vector variety $\mathcal{S}(\mathbf{R})$ of the hyperquiver in Figure \ref{fig:period-n-representation} computed in Macaulay2. In all cases, $\mathcal{S}(\mathbf{R})$ was zero-dimensional and the degree matched the conjectured formula \eqref{eq:number-of-n-periodic-fixed-points}. Dashes indicate computations not completing on time.}\label{tab:n-periodic-orbit}
\end{table}

==> figures/noSingularVectors.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.145\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Cropped0.pdf}
         \caption{}
         \label{noSingularVectors1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Cropped1.pdf}
         \caption{}
         \label{noSingularVectors2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Cropped2.pdf}
         \caption{}
         \label{noSingularVectors3}
     \end{subfigure}
        \caption{Quivers with empty singular vector varieties}
        \label{noSingularVectorQuivers}
\end{figure}
